AR-1-to-3: Single Image to Consistent 3D Object Generation via Next-View Prediction

Novel view synthesis (NVS) is a cornerstone for image-to-3d creation. However, existing works still struggle to maintain consistency between the generated views and the input views, especially when there is a significant camera pose difference, leading to poor-quality 3D geometries and textures. We attribute this issue to their treatment of all target views with equal priority according to our empirical observation that the target views closer to the input views exhibit higher fidelity. With this inspiration, we propose AR-1-to-3, a novel next-view prediction paradigm based on diffusion models that first generates views close to the input views, which are then utilized as contextual information to progressively synthesize farther views. To encode the generated view subsequences as local and global conditions for the next-view prediction, we accordingly develop a stacked local feature encoding strategy (Stacked-LE) and an LSTM-based global feature encoding strategy (LSTM-GE). Extensive experiments demonstrate that our method significantly improves the consistency between the generated views and the input views, producing high-fidelity 3D assets.

==> images/abl_ratio.tex <==
\begin{figure}[t]
  \centering
  \footnotesize
  \centering
  \includegraphics[width=0.8\linewidth]{images/files/abl_ratio.pdf}
  % \fbox{\rule[-.5cm]{0cm}{4.5cm} \rule[-.5cm]{5cm}{0cm}}
  \vspace{-7pt}
  \caption{\small Performance VS. Efficiency at different sampling ratios of the local features in the \nameoflocalmodule{} strategy.}
  \vspace{-10pt}
  \label{fig:abl_ratio}
\end{figure}

==> images/gallery.tex <==




% \twocolumn[{%
%     \renewcommand\twocolumn[1][]{#1}%
%     \maketitle
%     \vspace{-40pt}
%     \begin{center}
%       \captionsetup{type=figure}   
%       \footnotesize
%       % \fbox{\rule{0pt}{2.36in} \rule{0.9\linewidth}{0pt}}
%        \includegraphics[width=0.99\linewidth]{images/files/teaser.png}
%        \vspace{-13pt}    
%       \captionof{figure}{
%         Examples of high-quality 3D asset gallery generated by our \nMethod{} model.
%         % 
%         See the supplementary materials for more results.
%       }
%       \label{fig:gallery}
%       \vspace{3pt}    
%     \end{center}%
% }]  


\twocolumn[{%
    \renewcommand\twocolumn[1][]{#1}%
    \maketitle
    \vspace{-39pt}
    \begin{center}
      \captionsetup{type=figure}   
      \footnotesize
      % \fbox{\rule{0pt}{2.36in} \rule{0.9\linewidth}{0pt}}
       \includegraphics[width=0.95\linewidth]{images/files/teaser.png}
       \vspace{-13pt}    
      \captionof{figure}{
        Examples of high-quality 3D asset gallery generated by our \nMethod{} model.
        % 
        See \secref{subsec:quali} for more visualization results.
      }
      \label{fig:gallery}
      % \vspace{0.1pt}    
    \end{center}%
}]  

==> images/global.tex <==
\begin{wrapfigure}{r}{0.5\textwidth}
  \setlength{\abovecaptionskip}{2pt}
  % \vspace{-10pt}
  \centering
  % \includegraphics[width=0.95\linewidth]{block.pdf}
  \fbox{\rule[-.5cm]{0cm}{4.5cm} \rule[-.5cm]{5cm}{0cm}}
  \caption{\small xxx.}
  % \vspace{-15pt}
  \label{fig:global}
\end{wrapfigure}

==> images/mos.tex <==


\begin{figure}[!ht]
    \centering
    % \vspace{-0.2cm}
    % \vspace{-5pt}
    
    \includegraphics[width=0.95\linewidth]{images/files/mos.pdf}
    % \begin{overpic}[width=0.8\linewidth]{images/files/intro.pdf}
    % \put (10,32){{input view}
    % % \put (60,32){{\color{white}{\camsubset Subset}}}
    %  % 
    % % \put (-2,25){\rotatebox{90}{GT}}
    % % \put (-2,12){\rotatebox{90}{Butterfly}}
    % % \put (-2,4){\rotatebox{90}{Bird}}
    % \end{overpic}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    \vspace{-5pt}
    \caption{multi-object scenes.}
    \label{fig:mos}
    % \vspace{-10pt}
\end{figure}

==> images/suppl_ito3d.tex <==

\begin{figure*}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/files/supp_ito3d.pdf}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    \vspace{-3pt}
    \caption{Visualization results of the proposed \nMethod{} model on more image-to-3d examples.}
    \label{fig:suppl_ito3d}
    \vspace{-10pt}
\end{figure*}

==> images/suppl_view_syn_humanoid.tex <==


\begin{figure*}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/files/supp_view_sync_humanoid.pdf}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    % \vspace{-7pt}
    \caption{
    Visualization results of the proposed \nMethod{} model on novel view synthesis of humanoid-object examples.}
    \label{fig:suppl_view_syn_humanoid}
    % \vspace{-10pt}
\end{figure*}

==> images/suppl_view_syn_mo.tex <==


\begin{figure*}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/files/supp_view_sync_mo.pdf}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    \vspace{-3pt}
    \caption{
    Visualization results of the proposed \nMethod{} model on novel view synthesis of multi-object examples.}
    \label{fig:suppl_view_syn_mo}
    \vspace{5pt}
\end{figure*}

==> images/suppl_view_syn_word.tex <==


\begin{figure*}[t]
    \centering
    \footnotesize
    \includegraphics[width=0.98\linewidth]{images/files/supp_view_sync_word.pdf}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    % \vspace{-7pt}
    \caption{
    Visualization results of the proposed \nMethod{} model on novel view synthesis of word-object examples.}
    \label{fig:suppl_view_syn_word}
    \vspace{10pt}
\end{figure*}

==> images/wos.tex <==


\begin{figure}[!ht]
    \centering
    % \vspace{-0.2cm}
    % \vspace{-5pt}
    
    \includegraphics[width=0.96\linewidth]{images/files/wos.pdf}
    % \begin{overpic}[width=0.8\linewidth]{images/files/intro.pdf}
    % \put (10,32){{input view}
    % % \put (60,32){{\color{white}{\camsubset Subset}}}
    %  % 
    % % \put (-2,25){\rotatebox{90}{GT}}
    % % \put (-2,12){\rotatebox{90}{Butterfly}}
    % % \put (-2,4){\rotatebox{90}{Bird}}
    % \end{overpic}
    % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{13cm}{0cm}}
    \vspace{-5pt}
    \caption{word-object scenes.}
    \label{fig:wos}
    % \vspace{-10pt}
\end{figure}

==> sec/0_abstract.tex <==
\begin{abstract}
    
    % abstract
    % 1 background - why this topic
    %(2 Insight/observation) - challenge?
    % 3  - your motivation
    % 4 method - propose xxx
    % 5 details - specifically, whats you methods
    % 6 Experimental results - xx
    %
    
    % \todo{
    % Multi-view synthesis serves as a fundamental component in creating high-quality 3D assets.
    % % 
    % We observe that the existing works represented by the Zero123 series typically struggle to maintain cross-view consistency, especially when handling views with significantly different camera poses.
    % % 
    % To overcome this challenge, we present \nMethod{}, a new paradigm to progressively generate the target views in an autoregressive manner.
    % %
    % Rather than producing multiple discrete views of a 3D object from a single-view image and a set of camera poses or multiple views simultaneously under specified camera conditions, \nMethod{} starts from generating views closer to the input view, which is utilized as contextual information to prompt the generation of farther views.
    % %
    % In addition, we propose two image conditioning strategies, termed as \nameoflocalmodule{} and \nameofglobalmodule{}, to encode previously generated sequence views and provide pixel-wise spatial guidance and high-level semantic information for the generation of current target views.
    % %
    % Extensive experiments on several publicly available 3D datasets show that our method can synthesize more consistent 3D views.
    % and produce high-fidelity 3D assets that closely mirror the input image.
    % %
    % Code and pre-trained weights will be open-sourced.}
    

    % 1. background - why this topic：多视角合成是创造高质量3D资产的基石。
    % 2. Insight/observation) - challenge：现有的方法在目标视角与输入视角的相机姿态相差较大时容易生成与输入视角不一致的目标视角，并且生成的目标视角之间也可能不一致，导致生成的3D物体质量较差。
    % 3：Propose/motivation: 我们认为造成这个问题的原因在于这些方法以同等优先级的方式生成不同相机姿态的目标视角，因为我们观察到与输入视角相距较近的目标视角容易生成，且具有高保真度。
    % 4. method: 受此启发，我们提出\nMethod{}，这是一个新的范式先生成与输入视角较近的视角，这些视角被进一步用作上下文信息以next-view prediction 的方式渐进式生成更远的目标视角。
    % 5. details. 具体来说，我们使用一个目前新视角合成常用的基于图像的扩散模型来生成每一步的新视角，这类模型包含一个局部条件策略和一个全局条件策略分别将输入图像的像素级空间特征和高层次语义特征作为注入到注意力机制中。 为了将已经生成的视角子序列编码成下一视角预测的条件，我们相应地设计了一个基于堆叠的局部特征编码模块Stack-LE和一个基于LSTM的全局特征编码模块LSTM-GE。
    % 6. Experimental results: 大量的实验证明我们的方法能够极大地提高生成的目标视角与输入视角以及目标视角之间的一致性，并且生成出高保真度的3D资产。
    % 1
    Novel view synthesis (NVS) is a cornerstone for image-to-3d creation.
    % 2
    However, existing works still struggle to maintain consistency between the generated views and the input views, especially when there is a significant camera pose difference, leading to poor-quality 3D geometries and textures.
    % 3
    We attribute this issue to their treatment of all target views with equal priority according to our empirical observation that the target views closer to the input views exhibit higher fidelity.
    % 4
    With this inspiration, we propose \nMethod{}, a novel next-view prediction paradigm based on diffusion models that first generates views close to the input views, which are then utilized as contextual information to progressively synthesize farther views.
    % 5
    % Specifically, we employ a widely-used diffusion model, which typically contains a local conditioning strategy and a global conditioning strategy to inject pixel-level spatial features and high-level semantic information from the input images into the attention mechanism, to generate the target views in each step.
    %
    To encode the generated view subsequences as local and global conditions for the next-view prediction, we accordingly develop a stacked local feature encoding strategy (\nameoflocalmodule{}) and an LSTM-based global feature encoding strategy (\nameofglobalmodule{}).
    %
    Extensive experiments demonstrate that our method significantly improves the consistency between the generated views and the input views, producing high-fidelity 3D assets.
    %
    % Code and pre-trained weights will be made publicly available.
    

    
    % Represented by Zero123 series of works, recent advancements in single-view 3D generation research have shown prominent progress by utilizing pre-trained 2D diffusion generation models.
    % %
    % These approaches either generate multiple discrete views of a 3D object from a single-view image and a set of camera poses or produce multiple views simultaneously under specified camera conditions.
    % %
    % However, it is hard to maintain consistency across different views and camera angles, especially for poses with large differences.
    % %
    % In this paper, we introduce \textbf{\nMethod}, a novel paradigm to generate multiview images according to the input single image with significantly improved detail consistency. We achieve this by designing a novel auto-regressive scheme where novel views are generated based on previous views.
    % % for progressively generating target views in an autoregressive manner.
    % %
    % The core of our method is first to generate views closer to
    % the input view, which is utilized as contextual information to prompt the generation of farther views.
    % %
    % To this end, we propose two image conditioning strategies, termed as \textbf{\nameoflocalmodule{}} and \textbf{\nameofglobalmodule{}}, to encode the sequence views.
    % %
    % Particularly, \nameoflocalmodule{} encodes the previously generated views into a stack embedding, which is employed as a local condition to modify the key and value matrices of the self-attention layers for denoising the target views of the current step.
    % %
    % Meanwhile, \nameofglobalmodule{} divides the previously generated views into two groups based on their elevations, whose feature vectors are encoded by two LSTM modules into high-level semantic information for global conditioning.
    % %
    % Extensive experiments on benchmark datasets show that our method can synthesize more consistent 3D views and produce high-quality 3D assets that closely mirror the given image.
    % %
    % The code will be made publicly available.
    
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}\label{sec:intro}
\vspace{5.5pt}
% 背景，现状，问题
Synthesizing 3D objects from a single-view image has been a fundamental and enduring research in both computer vision and graphics communities.
%
This task is challenging, as it not only involves reconstructing the visible regions of a 3D object but also necessitates extrapolating the invisible parts.
%
To address these challenges, researchers have sought to synthesize novel views~\cite{qian2023magic123,chen2023cascade,long2024wonder3d,liu2024one} with the powerful priors of diffusion models, which have achieved remarkable success in image generation~\cite{rombach2022high,peebles2023scalable,li2024photomaker,zhou2024storydiffusion}.

Existing approaches can be broadly categorized into two distinct paradigms.
%
To be specific, the methods represented by Zero123~\cite{liu2023zero} fine-tune pre-trained diffusion models on $<$\emph{input\_view, camera\_pose, output\_view}$>$ triplets of 3D renders and generate multiple discrete views of a 3D object based on a single-view image and a set of camera poses.
%
On another line, Zero123++~\cite{shi2023zero123++} and its follow-ups~\cite{li2023instant3d,tang2024lgm,xu2024instantmesh,liu2024oneplus} consider the independence of new views specified by different camera poses.
%
They utilize diffusion models to generate multiple views simultaneously by merging all target views with specified camera poses into a grid image for joint distribution modeling.
%
Despite their success in many scenarios, these methods remain prone to synthesizing new views inconsistent with the input image, especially when there is a large gap between their camera poses, 
as illustrated in the bowls and shoes of \figref{fig:intro}.

\myinputfig{intro}



% 解决问题的思路
A fundamental reason for this issue is that these methods generate novel views for all camera poses in an equally prioritized manner.
%
We argue that novel views with camera poses closer to the input view should be generated first in that they usually exhibit substantially higher generation fidelity, whereas those with larger pose variations present greater challenges, as shown in \figref{fig:intro1}.
%
To this end, we rethink the way to generate consistent views and present \nMethod{}, a novel paradigm to progressively generate all target views, with the closer views generated first serving as contextual information to generate the farther view.


% 我们的方法
Our methodology follows the 3$\times$2 grid image generation strategy proposed by Zero123++~\cite{shi2023zero123++}.
% %
% In particular, the 6 target camera poses consist of interleaving elevations of $20^{\circ}$ downward and $-10^{\circ}$ upward, combined with azimuths that start at $30^{\circ}$ and increase by $60^{\circ}$ for each pose.
%
It is noteworthy that there exists a potential sequential relationship between these six target views, where the adjacent rows of views in the grid share identical elevation angles and a fixed azimuth interval of $120^{\circ}$.
%
This sequential nature enables our \nMethod{} to start from generating the first row views based on the input view and gradually generate the remaining row views in an autoregressive fashion.
% %
% Given a source image, \nMethod{} starts by generating the first row views of the $3 \times 2$ grid, and gradually generates the remaining row views in the subsequent steps with a fixed row azimuth interval of $120^{\circ}$ for each step.
%
At each iteration step, the target views from two different camera elevations can exchange information, and the views generated in the previous steps are utilized as references to generate current views.
% %
% To this end, we develop a conditional feature encoding scheme for both the image local conditioning and global conditioning of the diffusion models.

To encode partially generated sequence views and provide references for the next views, we develop two image conditioning strategies, \ie \nameoflocalmodule{} and \nameofglobalmodule{}, for local conditioning and global conditioning of the diffusion models respectively.
%
In the \nameoflocalmodule{} strategy, the denoising UNet model encodes the previously generated views into a stack embedding, which is employed as pixel-wise spatial guidance to modify the key and value matrices of the self-attention layers for denoising the target views of the current step.
%
In \nameofglobalmodule{}, the view subsequence is divided into 
two groups according to the elevation, whose feature vectors are encoded by two LSTM modules for high-level semantic conditions of current views.




% % 结果
We evaluate the performance of our \nMethod{} paradigm on a 3D benchmark dataset, \eg Objaverse~\cite{deitke2023objaverse}, and two out-of-domain datasets, \ie Google Scanned Objects~\cite{downs2022google}, and OmniObject3D~\cite{wu2023omniobject3d}.
%
By introducing the autoregressive manner coupled with the proposed \nameoflocalmodule{} and \nameofglobalmodule{} strategies into multi-view diffusion models, our \nMethod{} enables consistent and accurate novel view synthesis, resulting in high-quality 3D assets, as shown in \figref{fig:gallery}.
%
The experimental results also demonstrate the superiority of our \nMethod{} compared to cutting-edge new view synthesis methods and image-to-3d methods.


\myinputfig{intro1}

% 总结
Our contributions can be summarized as follows:
\begin{itemize}
    \item We propose \nMethod{}, an autoregressive next-view prediction framework for 3D object generation, which can generate target views from near to far progressively.
    % 
    \item We design \nameoflocalmodule{} and \nameofglobalmodule{} strategies to encode the partially generated sequence views and provide local and global conditions for the diffusion models.
    %
    \item Extensive quantitative and quantitative experiments on large-scale 3D datasets demonstrate that our approach can generate more consistent 2D multi-view images than previous works and produce high-quality 3D assets.
\end{itemize}

==> sec/2_relatedwork.tex <==
\section{Related Work}
\subsection{2D Diffusion Models for 3D Generation}
Diffusion Models~\cite{ho2020denoising,rombach2022high,peebles2023scalable,black2024flux} pre-trained on large-scale 2D datasets have demonstrated remarkable performance in generating high-quality images and powerful zero-shot generalization.
%
In recent years, significant effort has been consecutively devoted to transferring such merits of 2D diffusion models to 3D generation.

%
DreamFusion~\cite{poole2022dreamfusion}, SJC~\cite{wang2023score}, and Fantasia3D~\cite{chen2023fantasia3d} propose to distill the knowledge of a pre-trained 2D diffusion model by feeding the rendered views to it and performing per-shape optimization but suffer from artifacts such as over-saturated colors and the ``multi-face'' problem.
%
Zero123~\cite{liu2023zero} pioneers an open-world single-image-to-3D framework, in which diffusion models are fine-tuned to synthesize new views conditioned on an input view and a set of discrete camera poses.
% %
ImageDream~\cite{wang2023imagedream} adopts world camera coordination as in MVDream~\cite{shi2023mvdream} to recover 3D geometries.
%
Magic123~\cite{qian2023magic123} combines the 3D prior of Zero123 and the 2D prior of the stable diffusion model together to enhance the quality of generated 3D meshes.
%
One-2-3-45~\cite{liu2024one} uses Zero123 to generate multi-view images, which are lifted to 3D space to assist in the generation of 3D meshes.
%
Several approaches like Consistent123~\cite{lin2023consistent123} and MVD-Fusion~\cite{hu2024mvd}, improve Zero123 by incorporating additional priors, \ie boundary and depth.
%
Besides, more and more attention has been drawn to enforce consistency between the generated multiple views.
%
SyncDreamer~\cite{liu2023syncdreamer} adopts a 3D-aware attention mechanism to correlate the corresponding features across different views.
%
MVDiffusion~\cite{Tang2023mvdiffusion} generates multi-view images in parallel through the weight-sharing multi-branch UNet with shared weights and correspondence-aware attention. 
%
More recently, Cycle3D~\cite{tang2024cycle3d} and Free3D~\cite{zheng2024free3d} simultaneously generate multiple views to model their joint distribution.
%
Zero123++~\cite{shi2023zero123++} further proposes a strategy of tiling six target views surrounding the 3D object into a grid image.
%
This strategy has been successively adopted by follow-up works such as One-2-3-45++~\cite{liu2024oneplus}, Instant3D~\cite{li2023instant3d}, and InstantMesh~\cite{xu2024instantmesh}.
%

In contrast to these methods heavily relying on the 2D diffusion priors, our \nMethod{} inspired by human thinking also pays attention to the contextual information of the current object.
%
The method most similar to ours is Cascade-Zero123~\cite{chen2023cascade}.
%
It first uses a multi-view diffusion model to generate many extra views, which, along with the input image, are then fed into another diffusion model to produce a specific target view.
%
Different from this method, our \nMethod{} takes the relationship between the target views and the input image into account and utilizes a diffusion model to establish the potential sequence between them.
% %
% Given the target views closer to the input image are easier to generate, \nMethod{} gradually generates all target views from near to far in an autoregressive manner, in which the views generation of each step could be assisted by the views generated in earlier steps.


\subsection{Autoregressive Generation}

The autoregressive scheme, commonly employed in time series analysis and prediction, operates on the fundamental principle that the current value in a sequence can be explained by its preceding values.
%
Based upon this technology, researchers have developed a series of classical sequential modeling methods~\cite{hochreiter1997long,shi2015convolutional,vaswani2017attention,ma2023towards}.
%
In recent years, there has been a growing interest in extending such an autoregressive fashion to various communities.


PixelRNN~\cite{van2016pixel} is one of the pioneering methods to generate high-quality images with intricate details by modeling pixel dependencies.
%
VQ-VAE~\cite{van2017neural} revolutionizes the learning of discrete representations by incorporating the codebook mechanism, enabling efficient encoding and decoding processes of images.
%
VQ-GAN~\cite{esser2021taming} adopts a transformer architecture to model serialized visual parts and introduces adversarial loss during the training process.
%
Parti~\cite{yu2022scaling} proposes a pathways autoregressive model treating the image generation as a sequence-to-sequence modeling to generate high-fidelity photorealistic images.
%
VAR~\cite{tian2024visual}, LlamaGen~\cite{sun2024autoregressive}, and Infinity~\cite{han2024infinity} scale image generation by incorporating multimodal large models.
%
In addition, some approaches~\cite{ruhe2024rolling,jin2024pyramidal,chen2025diffusion,voleti2024sv3d,zuo2024videomv} attempt to integrate diffusion models with the sequential strategy to achieve more temporally consistent video generation.
%
More recently, MeshGPT~\cite{siddiqui2024meshgpt}, MeshAnything~\cite{chen2024meshanything}, and MeshXL~\cite{chen2024meshxl} proposes to generate triangle faces in an autoregressive manner for artist-created 3D meshes.
%
TAR3D~\cite{zhang2024tar3d} and SAR3D~\cite{chen2024sar3d} quantify 3D latent representations, which are utilized to generate 3D objects with the next-token prediction strategy.


In this work, we observe the target views of Zero123++ can be divided into several steps with equidistant camera pose intervals, resulting in a potential sequential nature.
%
% As a result, we propose to autoregressively generate multiple novel views.


==> sec/3_method.tex <==
\section{Methodology}\label{sec:method}

\subsection{Preliminaries}
We introduce the preliminaries of Zero123++~\cite{shi2023zero123++}, the base multi-view diffusion model adopted in this work, which is beneficial for understanding the designs in \nMethod{}.

\myPara{Multi-View Generation.}
To achieve the modeling of the joint distribution between multiple new views, Zero123++ proposes to tile six target views with a $3 \times 2$ layout in a grid image.
%
Note that these target views are obtained from a fixed set of relative azimuth and absolute elevation angles.
%
Specifically, they consist of interleaving elevation angles of $20^{\circ}$ downwards and $-10^{\circ}$ upwards, combined with azimuth angles starting from $30^{\circ}$ relative to the input azimuth and incrementing by $60^{\circ}$ for each subsequent camera pose.

\myPara{Stable Diffusion.}
Zero123++ chose Stable Diffusion (SD) as the generative model since it is open-sourced and has been trained on various internet-scale image datasets.
%
The geometric priors that SD learns about natural images are utilized for novel view synthesis under the image and camera conditions.
% 
SD performs the diffusion process within the latent space of a pre-trained autoencoder whose encoder and decoder are denoted as $\mathcal{E}(\cdot)$and $\mathcal{D}(\cdot)$, respectively.
%
At the diffusion time step $t$, the objective for fine-tuning the denoiser UNet $\epsilon_{\theta}(\cdot)$ can be formulated as:
\begin{equation} 
   \mathcal{L} = \mathbb{E}_{z \sim \mathcal{E}(x),y,t,\epsilon \sim \mathcal{N}(0,I)}||\\ \epsilon - \epsilon_{\theta}(z_{t},t,c_{\theta}(y) ||\\_{2}^{2},
  \label{eq:zero123plusobj}
\end{equation}
where $x$ is the target grid image which is perturbed to a feature by Gaussian noise $\epsilon$, \ie $z_{t}$, and $c_{\theta}(y)$ represents the embedding encoded from the condition image $y$. 


\myPara{Image Condition.}
The image conditioning techniques in Zero123++, \ie $c_{\theta}(y)$, can be divided into local and global conditions. 
%
The former strategy is tailored for the pixel-wise spatial correspondence between the input and target views.
%
Specifically, it adopts a variant of the Reference Attention operation~\cite{zhang2023reference}, which runs the denoising UNet on the input image and appends the self-attention key and value matrices from it to the corresponding attention layers when denoising the target views.
%
Note that the Gaussian noise at the same level as the denoising input is added to the referring image so that the UNet can focus on the relevant features for denoising at the current noise level.
% \todo{
% To this end, Zero123++ adopts a variant of the Reference Attention operation~\cite{zhang2023reference}, which runs the denoising UNet on the input image and appends the self-attention key and value matrices from it to the corresponding attention layers when denoising the target views.}
%
In terms of the global conditioning strategy, the CLIP~\cite{radford2021learning} text embedding of an empty text is added with the CLIP image embedding of the input image multiplied by a trainable set of global weights to provide high-level semantic information for the cross-attention of the denoising UNet.

\myinputfig{overall}



\subsection{\nMethod}
Existing methods either generate multiple discrete viewpoints from a single input view and a set of camera poses, like Zero123~\cite{liu2023zero}, One-2-3-45\cite{liu2024one}, or simultaneously generate multiple views in a grid layout based on specified camera conditions, such as Zero123++~\cite{shi2023zero123++}, ImageDream~\cite{wang2023imagedream}.
%
Despite achieving excellent performance in many scenarios, these methods are still prone to generating several target views that exhibit geometric and textural inconsistencies with the input image.
%
We argue that their equal prioritization of all new views and the underutilization of contextual information of current objects during the generation process should be responsible for this issue.

%
The core of this work is to progressively generate target views in a next-view prediction fashion so that the closer views generated earlier can be used as supplementary information for the generation of the farther views.
%
\figref{fig:overall} shows the end-to-end architecture of our \nMethod{}.
%
In this work, we follow the paradigm of Zero123++ generating 6 specific camera conditional target views.
%
In contrast, our method generates these views step by step rather than all at once.
%
In addition, Zero123++ has demonstrated that generating multiple target views simultaneously contributes to accurately modeling the joint distribution of these views.
%
Therefore, each step in our generative strategy refers to a row of the $3 \times 2$ layout, containing two target views with different elevations and $60^{\circ}$ difference in azimuth.
%
Moreover, the difference in camera pose between adjacent steps is a fixed azimuth angle of $120^{\circ}$, which is suitable for the next view prediction scheme.
%
As a result, the different target views at each step can exchange information, and the target views generated in the previous steps can be utilized as extra conditions to generate the views for the current step.


We achieve such next-view prediction by designing two image conditional strategies that encode sequence view information to fine-tune the diffusion model.
%
These two strategies, denoted as Stacked Local Feature Encoding (\nameoflocalmodule{}) and Long Short-Term Global Feature Encoding (\nameofglobalmodule{}), correspond to the local and global image conditioning techniques in Zero123++, respectively.
%
The optimization objective can still be represented by \eqnref{eq:zero123plusobj}, and we will elaborate on our image conditional policy, \ie $c_{\theta}(y)$, in the subsequent \secref{subsec:local} and \secref{subsec:global}.

%
% 需要单独写一段，自回归生成的多视角后接一个训练好的LRM，生成3D物体 
Through multi-step autoregression, our \nMethod{} gradually generates 6 target views, which are fed to a sparse-view large reconstruction model to obtain a 3D object.
%
In this work, we choose the pre-trained InstantMesh~\cite{xu2024instantmesh} as our 3D reconstruction model, which encodes the multi-view images as triplane features via a transformer-based architecture~\cite{hong2023lrm,luo2024vscode} and predicts the point color and density for volumetric rendering by a multi-layer perceptron.


\subsection{Stacked Local Feature Encoding} \label{subsec:local}
% \myinputfig{local}
% \figref{fig:local}
In this subsection, we introduce how our method encodes the latent features of the input image and the generated partial target-view sequence as local conditions for the operation of Reference Attention to generate the target views of the current step. 
%
Note that the denoising UNet model is a multi-level architecture and the hidden dimensions may vary across different self-attention layers.
%
It is challenging to encode the latent features of the condition view sequence at these positions using a single network.
%
Considering that these reference features and the attention representations in self-attention layers come from the same positions in the U-Net network, sharing the same spatial and channel dimensions, we naturally thought of encoding them into a unified representation by stacking them along the spatial dimension.
%
This strategy offers two significant advantages: 
%
1) it can encode any number of reference features at the self-attention layer.
%
2) it allows the reference features to be directly fed into the attention module, enabling the reuse of weight parameters without any additional design required.
%
We term this local feature encoding strategy as \nameoflocalmodule{} whose details are shown in the bottom left corner of \figref{fig:overall}.

% \myinputfig{local}
Formally, at the $k$-th step of autoregression, with a total of $2k$-$1$ reference views, we aim to predict the $(2k)$-th and $(2k$+$1)$-th target views, where the variable $k$ ranges from 1 to 3.
%  
Following Zero123++~\cite{shi2023zero123++}, we first feed the referring views into the denoising UNet model separately and record their key/value matrices at the self-attention module.
%
% Following Zero123++~\cite{shi2023zero123++}, gaussian noise at the same level as the denoising input is added to the reference so that the UNet can focus on the relevant features for denoising at the current noise level.
% 
Then, we perform another forward pass with the U-Net to denoise the target views of the current step.
%
During this process, the records in each layer are stacked together to modify the key and value matrices in the self-attention module of the corresponding layer, which can be defined as:
\begin{equation} 
   s^{*}_{i} = \mathrm{Concat}([e^{1}_{i}, e^{2}_{i}, ..., e^{2k-1}_{i}, s_{i}]),
  \label{eq:local_att_kv}
\end{equation}
where $s_{i} \in \mathbb{R}^{B \times L \times D_{i}}$ denotes the key or value matrices of the $i$-th self-attention, and $e_{i}^{j}$ is the recorded embeddings of the $j$-th reference view.
%
Note that $B$, $L$ and $D_{i}$ are the batch size, token number, and dimension of the key /value matrices.
%
Further, we compute the self-attention as follows:
\begin{equation} 
   O_{i} = \mathrm{Attention}([Q_{i}, K^{*}_{i}, V^{*}_{i}]).
  \label{eq:local_att}
\end{equation}

% It is noteworthy that \nameoflocalmodule{} may encounter GPU burden issues when the sequence length becomes excessively long.
% %
% To alleviate this concern, we introduce a novel random sampling strategy inspired by recent works on video generation~\cite{zhou2024storydiffusion}.
% %
% Specifically, we retain all $L$ tokens of $e_{i}^{1}$ as they originate from the input image, and perform random sampling with a proportion of $\alpha$ on the $L$ tokens from each generated target view. 
% %
% When the $\alpha$ value is 0, \nameoflocalmodule{} degenerates into the original Reference attention; when $\alpha$ is 1, it is equivalent to using all tokens as in \eqnref{eq:local_att_kv}.
% %
% As far as the selection of $\alpha$, please refer to \secref{subsec:abl} for more details.


\subsection{Long Short-Term Global Feature Encoding} \label{subsec:global}
In this subsection, we present the details of encoding the CLIP features of the input images and the existing target-view sequence as global conditions, which provide high-level semantic information via cross-attention to generate the target views of the current step.
%
We empirically observe that the CLIP features of the conditional view sequence are vectors with the same channel dimension and 1D spatial dimensions.
%
In addition, they can be divided into two sub-sequences with an azimuthal angle spacing of $120^{\circ}$ based on their elevation angles.
%
Thus, it is well-suited to process such sequences with the Long Short-Term Memory (LSTM) Network~\cite{hochreiter1997long}.
%
Furthermore, this manner has two interesting merits, mitigating computational burden: 
% 
1) It can encode feature vectors from the conditional views into two vectors,  regardless of the number of views.
% 
2) The LSTM structure possesses a strong ability to model sequential representations while requiring fewer parameters.
%
This strategy is named as \nameofglobalmodule{}, and the diagrammatic details are shown in the bottom left corner of \figref{fig:overall}.



Given $2k$-$1$ conditional views at the $k$-th step of autoregression, we first send them to the image encoder of the CLIP model for their visual features, which are represented as $F \in \mathbb{R}^{B \times (2k-1) \times D}$.
%
Then, we partition these features into two groups according to the elevation angles of their respective views.
%
Note that the feature of the input image is a special case, which is included in both groups.
%
We denote the two grouped features as $F_{1} \in \mathbb{R}^{B \times k \times D}$ and $F_{2} \in \mathbb{R}^{B \times k \times D}$, and feed them to two separate LSTM modules.
%
Next, the hidden states of the $k$-th step of the two LSTM modules, \ie $h_{l}^{k}$, are selected as their respective outputs, \ie, $I_{l}$.
%
This process can be formulated as follows:
%
\begin{equation} 
  I_{l} = \mathrm{LSTM}_{l}([F_{l}, (h_{l}^{0}, c_{l}^{0})]), \quad l \in \{0, 1\}
 \label{eq:global_lstm}
\end{equation}
where $h_{l}^{0}$ and $c_{l}^{0}$ are the hidden state and cell state, respectively, both initialized as zero vectors.
%
Finally, the outputs of the two LSTM modules are concatenated together along the channel dimension, followed by an MLP layer and a trainable set of global weights $W \in \mathbb{R}^{77 \times 1}$, to form global embeddings for the cross-attention of the denoising UNet:
%
\begin{equation} 
  T = W \cdot \mathrm{MLP}(\mathrm{Concat}([I_{0}, I_{1}])). \quad T \in \mathbb{R}^{B \times 77 \times D}
 \label{eq:global_concat}
\end{equation}
%
Note that we remove the CLIP embedding of empty text from the original global condition, as empirical observations indicate its negligible impact on the final results.



==> sec/4_exp.tex <==
\section{Experiments}\label{sec:experiment}
\myinputfig{view_syn}

\myinputfig{show}
\subsection{Experiment Setup}\label{sec:exp_setting}

\myPara{Datasets.}
We conduct experiments on the most popular benchmarking 3D dataset, \ie Objaverse~\cite{deitke2023objaverse}, along with two out-of-domain datasets, \ie  Google Scanned Objects (GSO)~\cite{downs2022google} and OmniObject3D (Omni3D)~\cite{wu2023omniobject3d}.
%
Following the filtering principle in previous works~\cite{zhang2024tar3d,li2025triposg}, we obtain about 210,000 geometry objects from the Objaverse dataset with a 3D mesh capacity of 800,000. 
%
We pick out 300 objects covering various categories to evaluate the performance of the methods, and the remaining samples are used for training.
%
Moreover, we also randomly select 300 samples each from both GSO and Omni3D to ensure a fair evaluation of the methods involved in this paper.

%
Following the protocol of Zero123++~\cite{shi2023zero123++}, we render 7 images for each object, including an input image and 6 target images.
%
To be specific, an elevation angle ranging from $-20^{\circ}$ to $45^{\circ}$ and an azimuth angle ranging from $0^{\circ}$ to $360^{\circ}$ are randomly sampled to render the input image.
%
The camera poses of the 6 target images involve interleaving absolute elevations of $20^{\circ}$ and $-10^{\circ}$, paired with azimuths relative to the input image that start at $30^{\circ}$ and increase by $60^{\circ}$ for each pose.
%
Besides, all rendered images are set to a white background to ensure that the diffusion model produces images of this nature, thereby avoiding the trouble of removing the background when reconstructing 3D objects.
%
We will open-source these rendered images in our project.

\myPara{Evaluation.}
We evaluate the performance of the methods in two critical dimensions, \ie 2D visual fidelity and 3D geometric accuracy.
Specifically, we compare the novel views generated by multi-view diffusion models or rendered from synthesized 3D meshes with the ground truth views.
%
Following image comparison~\cite{lin2023consistent123,chen2023cascade,xu2024instantmesh}, we report four popular metrics, including Peak Signal-to-Noise Ratio (PSNR), Perceptual Loss(LPIPS)~\cite{zhang2018unreasonable}, Structural Similarity (SSIM)~\cite{wang2004image}, and CLIP-score~\cite{radford2021learning}.
%
We also compare the surface points randomly sampled from the
generated 3D meshes with those from ground-truth meshes, in which the chamfer distance (CD) value and the F-Score with a threshold of 0.02 are employed as metrics.



\myPara{Implementation Details.}
We train \nMethod{} on the render images from about 210K objects of the Objaverse dataset for 150k steps with a total batch size of 32 on 8 NVIDIA A100 (80G) GPUs.
%
The learning rate is initialized as $1e$-$5$ and changes every 25k steps in a cycle, along with the AdamW optimizer~\cite{loshchilov2019decoupled} and CosineAnnealingWarmRestarts scheduler~\cite{loshchilov2016sgdr}.
%
We randomly select a $k$ from $\{1, 2, 3 \}$ to build the autoregressive pattern, where the first $2k$-$1$ views form the conditional images and the following two views make up the target views.
%
We resize the size of the conditional images to a value between 128 and 512 so that the model is capable of adjusting to different input resolutions and producing more clear images.
%
Meanwhile, we resize each target view to 320, thereby the size of the grid image during the autoregressive process is 320$\times$640. 
%
In addition, we employ the linear noise schedule and v-prediction loss in Zero123++~\cite{shi2023zero123++} rather than the alternatives in the Stable Diffusion model~\cite{rombach2022high}.
%
During the inference stage, taking the input image as initialization, our \nMethod{} generates all target views in three steps, as shown in \figref{fig:show}.



\myinputfig{ito3d}
\subsection{Qualitative Results} \label{subsec:quali}

We perform qualitative experiments on novel view synthesis and image-to-3d on a wide range of 3D objects.
%
To highlight the advantages of our \nMethod{} method in contextual reasoning and zero-shot generalization, we adopt input views with a certain degree of offset relative to the frontal views of 3D samples.
%
We also provide more visualization results in the supplementary material.


\myPara{Novel View Synthesis.}
\figref{fig:view_syn} shows the synthesized views of our \nMethod{} and recent popular methods in multi-view generation, including Zero123-XL~\cite{liu2023zero}, SyncDreamer~\cite{liu2023syncdreamer}, Zero123++~\cite{shi2023zero123++}, One-2-3-45~\cite{liu2024one}.
%
Note that Zero123-XL is an enhanced Zero123 model pre-trained on the Objaverse-XL dataset, and the open-source project of One-2-3-45 also employs this Zero123 version to generate the 8 views for its first stage.
%
We utilize the elevation estimation implements of One-2-3-45 for the necessary elevation estimation procedures in Zero123-XL and SyncDreamer.
%
Among these difficult-to-maintain consistency scenes, some methods produce multiple inconsistent novel views, as shown in the bench results of Zero123++ and the cartoon figure of Zero123-XL. 
%
Some approaches may even be confused and generate new views that differ significantly from the input image, as shown in the bench predictions of SyncDreamer and the four-wheeled beds of One-2-3-45.
%
In contrast, our \nMethod{} is able to capture texture details of 3D objects and synthesize consistent multi-view images, which can be attributed to the full utilization of contextual information.



\myPara{Image-to-3D.}
Based on the synthesis of more consistent multiple views, our \nMethod{} can further generates high-quality 3D objects, as shown in \figref{fig:show}.
%
We also compare it with five cutting edge image-to-3d approaches, \ie SyncDreamer~\cite{liu2023syncdreamer}, InstantMesh~\cite{xu2024instantmesh}, One2345++~\cite{liu2024oneplus}, TripoSR~\cite{tochilkin2024triposr}, and Unique3D~\cite{wu2024unique3d}.
%
Note that the visual comparisons contain the pure geometries (left) and textured renderings (right) for each mesh generated by these methods.
%
As depicted in \figref{fig:ito3d}, our \nMethod{} can generate 3D meshes with a consistent appearance and plausible geometry under limited input view information.
%
Nevertheless, it is a real struggle for the counterparts to achieve this.
%
For example, InstantMesh and One2345++ tend to generate an additional storage cabinet for the desk. 
%
We speculate that this is due to their excessive reliance on the symmetry prior of diffusion models during the generative process of new views, with less consideration for the contextual information of the object itself.
%
Although SyncDreamer does not generate additional components, the desk it produces exhibits significant geometric deformations.
%
We find that the reason stems from the inconsistency among the 16 views generated by its diffusion model, which is employed to reconstruct the 3D object.
%
Unlike these approaches, our \nMethod{} effectively utilizes the contextual information of the object itself from nearby to distant during the autoregressive generation of all target views.
%
As a result, our method can achieve excellent performance in image-to-3D generation.




\subsection{Quantitative Results}

\myinputtab{quan}
We conduct quantitative studies on the two out-of-domain datasets, \ie GSO and Omni3D, to evaluate the performance of our \nMethod{} and other \sArt methods fairly.
%
Specifically, all candidate approaches are fed the same input images to generate 3D assets.
%
We render 20 views with 224$\times$224 resolution for each mesh to perform the 2D evaluation.
%
As far as the 3D evaluation, we uniformly sample 16K points from the mesh surfaces in an aligned
cube coordinate system of [-1,1]$^3$.
%
As shown in \tabref{tab:quan}, our \nMethod{} surpasses other cutting-edge methods across all metrics.
%
These results further demonstrate the superiority of our \nMethod{} in 3D asset creation.

% We also quantitatively evaluate the performance of our \nMethod{} and other \sArt methods on two out-of-domain datasets.
% %
% For each 3D sample, these methods generate six target views according to the settings of Zero123++~\cite{shi2023zero123++}.
% %
% For the methods that do not support changing the elevation angle, \eg  SyncDreamer, we first generate 3D meshes following their default pipelines and then use Blender to render the views of these camera poses. 
% %
% As shown in \tabref{tab:quan}, our \nMethod{} surpasses other cutting-edge methods across all metrics by a large margin.
% %
% These results further demonstrate the superiority of our \nMethod{} over
% existing methods on the multi-view generation of 3D objects.

\subsection{Ablative Study} \label{subsec:abl}
% In this subsection, we conduct ablative studies and analysis to investigate the effectiveness of our designs in \nMethod{}, including the sequence order in autoregressive generation, the sampling ratio in \nameoflocalmodule{}, and the encoding strategy in \nameofglobalmodule{}.

We conduct ablative experiments on the 300 objects excluded from training to examine the effectiveness of our key designs in the proposed \nMethod{} framework. 

\myinputtab{abl_components}


\myinputtab{abl_order}

\myPara{Ablation on Image Conditioning Components.}
%
Starting from the Zero123++ baseline, we first incorporate \nameoflocalmodule{} strategy, then \nameofglobalmodule{} independently, and finally integrate both strategies.
%
As shown in \tabref{tab:abl_components}, they individually contribute to performance improvements, and their combined integration produces a greater improvement compared to the baseline method.
%
These results demonstrate both the effectiveness of the two image conditioning strategies and the significant contribution of our next-view prediction in advancing the accuracy of novel view synthesis.

\myPara{Ablation on Different Sequence Orders.}
We define the sequence order from near to far in terms of camera poses relative to the input viewpoint as the normal order.
%
We also provide two variants of the sequence order, \ie reverse order and random order, to generate target views.
%
To be specific, the reverse order refers to the view sequence whose cameras move from far to near relative to the input view.
%
Meanwhile, the random order places the middle row of the $3 \times 2$ grid layout as the first position, followed by the remaining two rows.
%
As shown in \tabref{tab:abl_order}, our normal order achieves the best performance, while the random sequence performs the worst, demonstrating the effectiveness of modeling the target views in a sequential manner.
%
Note that the reverse order achieves a similar performance to our normal order.
%
We believe the reason for this is that the reversed sequence under Zero123++ setting can be seen as the camera moving from near to far in another circle direction, as the camera moves in a circular motion around the 3D object.





\myPara{Encoding Strategy of Global Feature Sequence.}
% Our \nameofglobalmodule{} employs two LSTM modules to encode the global features of conditional view sequence.
%
To highlight the effectiveness of our \nameofglobalmodule{} for global feature encoding of view sequence, we design a matrix multiplication (`matmul') variant to encode these features.
%
Specifically, we stack these features into a matrix with shape $\mathbb{R}^{(2k-1) \times D}$.
%
Meanwhile, we repeat the trainable weights in global condition $(2k$-$1)$ times to obtain a matrix with shape $\mathbb{R}^{77 \times (2k-1)}$.
%
We multiply these two matrices to obtain a new matrix with shape $\mathbb{R}^{77 \times D}$, which is utilized as the key and value matrix for the cross-attention mechanism of the denoising UNet.
%
As depicted in \figref{fig:abl_enc}, with the incorporation of extra contextual information, the `matmul' variant can generate more consistent and high-quality multi-view images compared to the baseline method, \ie Zero123++.  
%
Nevertheless, this variant may lead to bias in the global semantic understanding of 3D objects, such as the shapes of the book sample.
%
In contrast, our strategy can generate multi-view images that are faithful to the shape and texture of objects in the input views.
%
These experiments indicate the LSTM proposal can more
effectively capture the high-level semantic information of the 3D objects.


\myinputfig{abl_enc}      % 图像对比








==> sec/5_conclusion.tex <==
\section{Conclusions}
In this paper, we present \nMethod{}, a next-view prediction paradigm that starts from the input image and progressively generates target views from near to far.
%
At each step of the autoregressive process, the previously generated views are employed as contextual information to facilitate the generation of the current target views.
%
The experimental results demonstrate that our method generates new view images and 3D objects that are more consistent with the input images compared with the existing approaches generating multi-view images discretely or simultaneously.
% %
% To accomplish such autoregression, we propose two image conditional strategies, \ie \nameoflocalmodule{} and \nameofglobalmodule{}, that encode sequence view information to fine-tune the denoising UNet model.
% %
% Particularly, \nameoflocalmodule{} encodes the latent features of conditional images as a stacked embedding to modify the key and value matrices of the self-attention mechanism in the UNet.
% %
% Meanwhile, \nameofglobalmodule{} adopts two LSTM modules to encode the CLIP features of conditional images into two feature vectors, which are concatenated together to provide high-level semantic information via cross-attention for the generation of the current target views.
%
% We hope our \nMethod{} could become one of the base multi-view generative models for image-to-3D, and such an autoregressive idea will inspire future works.

